ExWarp: Extrapolation and Warping-based Temporal Supersampling for High-frequency Displays

High-frequency displays are gaining immense popularity because of their increasing use in video games and virtual reality applications. However, the issue is that the underlying GPUs cannot continuously generate frames at this high rate -- this results in a less smooth and responsive experience. Furthermore, if the frame rate is not synchronized with the refresh rate, the user may experience screen tearing and stuttering. Previous works propose increasing the frame rate to provide a smooth experience on modern displays by predicting new frames based on past or future frames. Interpolation and extrapolation are two widely used algorithms that predict new frames. Interpolation requires waiting for the future frame to make a prediction, which adds additional latency. On the other hand, extrapolation provides a better quality of experience because it relies solely on past frames -- it does not incur any additional latency. The simplest method to extrapolate a frame is to warp the previous frame using motion vectors; however, the warped frame may contain improperly rendered visual artifacts due to dynamic objects -- this makes it very challenging to design such a scheme. Past work has used DNNs to get good accuracy, however, these approaches are slow. This paper proposes Exwarp -- an approach based on reinforcement learning (RL) to intelligently choose between the slower DNN-based extrapolation and faster warping-based methods to increase the frame rate by 4x with an almost negligible reduction in the perceived image quality.

==> methodology.tex <==
\section{Methodology}
\label{sec:methodology}
\subsection{Overview}
\label{sec:overview}
We propose to insert three new frames at time instances $t+0.25$, $t+0.5$, $t+0.75$ between any two consecutive frames $F_t$ and $F_{t+1}$. As mentioned in Section~\ref{sec:Introduction}, warping and extrapolation are two options for synthesizing these new frames. Based on these two algorithms, multiple scenarios are possible (refer to Figure~\ref{fig_overview}).  

%Now, we have two choices for the remaining two frames- warping and extrapolation. For the first frame $P_{t+0.25}$, extrapolation is not an option because if we start extrapolating frame $F_{t}$ at time $t$, the extrapolation takes at least $t+0.5$ time. So, the remaining choice to generate $P_{t+0.25}$ is warping $F_t$. We may use warping and extrapolation for $P_{t+0.75}$. If we use extrapolation, we need to finish extrapolating $P_{t+0.75}$ prior before $t+0.75$; we start extrapolating $P_{t+0.25}$ at time $t+0.25$. Since warping takes less time, we warp the latest frame $P_{t+0.25}$ instead of using $P_{t+0.5}$.

\begin{figure}[]
	\centering
	\includegraphics[width=0.99\columnwidth]{overview.pdf}
	\caption{Overview of the proposed system. $F_t$ and $F_{t+1}$ are two rendered frames. $W$ and $E$ stand for warping and extrapolation, respectively. $P_1$, $P_2$, and $P_3$ are predicted frame.}
	\label{fig_overview}
\end{figure}
\subsection{Problem Formulation}
\label{problem}
Given two rendered frames $F_t$ and $F_{t+1}$, our goal is to insert $n$ new frames between these two frames without using $F_{t+1}$, where $n$ $\in$ $[1,3]$. We represent these frames as $P_i$, where $i$ falls within the interval $[0,n]$ and the frame $P_i$ is displayed on the screen at time $t+(i/4)$. The value of $n$ depends on the algorithm used for generating $P_i$. We have two options - warping and extrapolation - we store them in a set A, denoted by $\{W, E\}$. 
 In the span of time from $t$ to $t+1$, we may have to choose an algorithm from set $A$ at most five times, denoted as $d_1$, $d_2$, $d_3$, $d_4$, and $d_5$, at $t$, $t+0.25$, and $t+0.5$ based on the current state of the system. The decision at time $t$, $d_1$, is whether to display the warped $F_1$ or wait for the extrapolated frame. Since the extrapolated frame would be available at time $t+0.5$, the last displayed frame i.e. $F_t$ remains on the screen; it also skips the decision at $t+0.25$. We show the complete flow based on various selections made at different time instances in Figure~\ref{flow}. Based on these five decisions, six scenarios for frames $P_i$s sre possible (refer to Table~\ref{pos_sce})

\begin{figure}[]
	\centering
	\includegraphics[width=0.99\columnwidth]{flow.pdf}
	\caption{Flow of the proposed approach. $d1$, $d2$ ,and $d3$ are the decisions taken at time $t$, $t+0.25$, and $t+5$, respectively. $W$ and $E$ stand for warping and extrapolation, respectively.}
	\label{flow}
\end{figure}



\begin{table}[]
\footnotesize
\begin{center}
\resizebox{0.99\columnwidth}{!}{
\begin{tabular}{| l |l | l| l| l|} 

\hline
\textbf{Scenario} &
$\mathbf{P_1}$ & $\mathbf{P_2}$ & $\mathbf{P_3}$ & \textbf{Frame rate}\\
&  &  & & \textbf{upsampling} \\ 
\hline\hline
$\mathbf{S_1}$ & $F_1$  & Extrapolated $F_1$  & Extrapolated $F_1$ & 2$\times$\\
 &  (No new frame)  &  &  (No new frame) &   \\ \hline
$\mathbf{S_2}$ & $F_1$   & Extrapolated $F_1$  & Warped $P_2$ & 3$\times$ \\
 & (No new frame) &  &  &   \\ \hline
$\mathbf{S_3}$ & Warped $F_1$ & Extrapolated $F_1$ & Extrapolated $P_1$ & 4$\times$\\  \hline
$\mathbf{S_4}$ & Warped $F_1$ & Extrapolated $F_1$ & Warped $P_2$ & 4$\times$\\  \hline
$\mathbf{S_5}$ & Warped $F_1$ & Warped $P_1$ & Extrapolated $P_1$ & 4$\times$\\  \hline
$\mathbf{S_6}$ & Warped $F_1$ & Warped $P_1$ & Warped $P_2$ & 4$\times$\\
\hline
\end{tabular}
}
\end{center}
%\caption{Details of the baseline system}
\caption{Possible scenarios based on the type of synthesized frames- $P_1$, $P_2$, and $P_3$}
\label{pos_sce}
\end{table}










==> motivation.tex <==
\section{Motivation}
\label{sec:Motivation}

